Counting Algebraic Curves with Tropical Geometry

Tropical geometry is a piecewise linear "shadow" of algebraic geometry. It allows for the computation of several cohomological invariants of an algebraic variety. In particular, its application to enumerative algebraic geometry led to significant progress. In this survey, we give an introduction to tropical geometry techniques for algebraic curve counting problems. We also survey some recent developments, with a particular emphasis on the computation of the degree of the Severi varieties of the complex projective plane and other toric surfaces as well as Hurwitz numbers and applications to real enumerative geometry. This paper is based on the author's lecture at the Workshop on Tropical Geometry and Integrable Systems in Glasgow, July 2011.

==> pics/bigpolygon_with_lattice <==
#FIG 3.2
Portrait
Center
Metric
A4 
100.0
Single
-2
1200 2
4 0 0 100 1 0 18.0 0.0 4 352.0 336.0 2025 2362 -2\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 1462 3037 0\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 1800 3712 1\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 2475 4162 2\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 3375 4612 2\001
4 0 0 100 1 0 18.0 0.0 4 352.0 336.0 5287 4612 -1\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 5625 3937 0\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 5287 3262 1\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 4837 2925 1\001
4 0 0 100 1 0 18.0 0.0 4 352.0 176.0 3825 2362 3\001
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4950 4500 60 60 4890 4440 5010 4560
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4500 4500 60 60 4440 4440 4560 4560
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4050 4500 60 60 3990 4440 4110 4560
1 1 0 2 0 0 100 1 20  6.40 1 0.0 5400 4050 60 60 5340 3990 5460 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4950 4050 60 60 4890 3990 5010 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4500 4050 60 60 4440 3990 4560 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4050 4050 60 60 3990 3990 4110 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3600 4050 60 60 3540 3990 3660 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3150 4050 60 60 3090 3990 3210 4110
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2250 3600 60 60 2190 3540 2310 3660
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 5
       1800 3150 2250 3600 1800 3150 1800 2700
       1800 3150
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2700 3600 60 60 2640 3540 2760 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3150 3600 60 60 3090 3540 3210 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3600 3600 60 60 3540 3540 3660 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4050 3600 60 60 3990 3540 4110 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4500 3600 60 60 4440 3540 4560 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 5400 3600 60 60 5340 3540 5460 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4950 3600 60 60 4890 3540 5010 3660
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4950 3150 60 60 4890 3090 5010 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4500 3150 60 60 4440 3090 4560 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4050 3150 60 60 3990 3090 4110 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3600 3150 60 60 3540 3090 3660 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3150 3150 60 60 3090 3090 3210 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2700 3150 60 60 2640 3090 2760 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2250 3150 60 60 2190 3090 2310 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 1800 3150 60 60 1740 3090 1860 3210
1 1 0 2 0 0 100 1 20  6.40 1 0.0 1800 2700 60 60 1740 2640 1860 2760
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2250 2700 60 60 2190 2640 2310 2760
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2700 2700 60 60 2640 2640 2760 2760
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       3150 2250 4500 2700 3150 2250
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4500 2700 60 60 4440 2640 4560 2760
1 1 0 2 0 0 100 1 20  6.40 1 0.0 4050 2700 60 60 3990 2640 4110 2760
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3600 2700 60 60 3540 2640 3660 2760
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3150 2700 60 60 3090 2640 3210 2760
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       3150 2250 4500 2700 3150 2250
1 1 0 2 0 0 100 1 20  6.40 1 0.0 3150 2250 60 60 3090 2190 3210 2310
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       2700 2250 1800 2700 2700 2250
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       2700 2250 1800 2700 2700 2250
1 1 0 2 0 0 100 1 20  6.40 1 0.0 2700 2250 60 60 2640 2190 2760 2310
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       2700 2250 1800 2700 2700 2250
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 5
       1800 3150 2250 3600 1800 3150 1800 2700
       1800 3150
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       3150 4050 2250 3600 3150 4050
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       3150 4050 4050 4500 3150 4050
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       4950 4500 4050 4500 4950 4500
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       5400 4050 4950 4500 5400 4050
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       5400 3600 5400 4050 5400 3600
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       4500 2700 5400 3600 4500 2700
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       3150 2250 4500 2700 3150 2250
2 3 0 2 0 0 100 1 -1  6.40 0 0 12 0 0 3
       2700 2250 3150 2250 2700 2250

